FirmUSB: Vetting USB Device Firmware using Domain Informed Symbolic Execution

The USB protocol has become ubiquitous, supporting devices from high-powered computing devices to small embedded devices and control systems. USB's greatest feature, its openness and expandability, is also its weakness, and attacks such as BadUSB exploit the unconstrained functionality afforded to these devices as a vector for compromise. Fundamentally, it is virtually impossible to know whether a USB device is benign or malicious. This work introduces FirmUSB, a USB-specific firmware analysis framework that uses domain knowledge of the USB protocol to examine firmware images and determine the activity that they can produce. Embedded USB devices use microcontrollers that have not been well studied by the binary analysis community, and our work demonstrates how lifters into popular intermediate representations for analysis can be built, as well as the challenges of doing so. We develop targeting algorithms and use domain knowledge to speed up these processes by a factor of 7 compared to unconstrained fully symbolic execution. We also successfully find malicious activity in embedded 8051 firmwares without the use of source code. Finally, we provide insights into the challenges of symbolic analysis on embedded architectures and provide guidance on improving tools to better handle this important class of devices.

==> Phison.tex <==
The first firmware we used is the Phison Firmware which was crafted by \cite{badusb} for the purposes of showing malicious behavior. The firmware initially enumerates itself as a mass storage device and later on can enumerate as an HID. After a predefined threshold count, it starts sending data from a saved script. Since, the device is at that point is recognized as a HID, the sent data is accepted as valid key strokes. The firmware worked on 8051 architecture. As a result we chose 8051 as our target architecture to begin analysis.

\paragraph{Query 1}
We start by looking for USB specific constants for to reason about Query 1. Using static analysis on the generated IRs we found instructions that use either one of the descriptors to load from. For each descriptor a set is kept that records the destination addresses where these descriptors get copied to. We took the intersection of these sets and found the possible set of EP0 address. In this case there was only one common element and the EP0 address was found to be 0xf1dc. Comparing with the source code we found that this was indeed the address of the FIFO in EP0. This enabled us to find the instruction where HID descriptor was being copied to EP0. We could reach the target in short time using Algorithm \ref{fig:algfindsym} to set symbolic regions for the analysis engines. The times shown in Table \ref{table:timingresults} is show the effectiveness of our algorithms in reaching Query 1 targets. When we do not apply Algorithm \ref{fig:algfindsym} the time to reach targets is highest. The combination of Algorithm \ref{fig:algfindsym} and domain specific constraining gives the best performance. When the size of symbolic memory region is reduced we automatically end up with fewer paths to go in. Since we determine the symbolic regions in a sound way we actually reach the target with lower number of paths to test. Also domain specific constraining further improves the performance. We restricted the path based two factors; speed change which does not affect our query and making sure to chose call to Get\_DESCRIPTOR function as the successor when the deciding switch statement comes. This pruning is sound for reachability testing because we combine domain specific knowledge. Using our optimizations we achieved maximum of 7.7x speed up compared to the fully symbolic version unconstrained execution for HID target.

\paragraph{Query 2}
To check for inconsistent data flow in the firmware using Algorithm \ref{fig:algcheckunexp}. Since we set all inputs to be symbolic there should only be symbolic data flowing to any output port. We look for constant data flows to endpoints. The EP0 found for Query 1 is used to calculate other endpoint addresses using constant offset. We were able to find constant data being copied to EP3.


==> llvmIRConcernsShort.tex <==
%\documentclass[10pt]{article}
%work in progress
%\begin{document}
\subsection{LLVM IR}
\noindent \paragraph{{\bf Assembly to IR:}} While {\tt LLVM IR} has the ability to represent most assembly operations into a sequence of {\tt IR} operations, it is designed for converting source code into {\tt IR}. Disassembled firmware does not explicitly contain all information easily available at the source level e.g. function boundaries are not as evident. This lack of information makes mimicking the hardware behavior troublesome. Implicit tasks done by the hardware have to be explicitly mentioned in {\tt IR}. Which tend to make the {\tt IR} much longer in terms of number of instructions. For example an instruction such as {\tt mov dest, src } copies the content of address {\tt src} to address {\tt dest}. In hardware terms, it can be a simple bus transaction between two memory locations. The operation is also dependent on the word size of the architecture. Register contents can not be affected by this instruction. So, while converting this {\tt mov} instruction into {\tt LLVM IR} there are a few things to consider. Data has to be read starting from {\tt src} address and of length determined by the word size. The read value has to be explicitly written to the {\tt dest} address. For instructions that affect the flags, explicitly each flag in {\tt IR} has to be set with the appropriate value. Flag setting cannot be determined by only the assembly instructions. Architecture dependent information is needed for this. For example, in 8051 architecture it's not just the arithmetic operations that affect carry flag, there are some bitwise rotate operations that can affect it too. Extensive knowledge of the instruction set architecture is required for this purpose.
%\end{document}


==> security.tex <==


\begin{figure}
\begin{algorithmic}[1]
\State {\bf FindCandidateHIDToEP0}($F$: Firmware)
\State $candConfDesc \gets \emptyset$
\For{each memory location $m \in F.AddressSpace$}
  \If{$m[0] = 0X39$}
      \State $candConfDesc \gets candConfDesc \cup \{m\}$
  \EndIf
\EndFor
\State $candHIDDesc \gets ...$
\State $targetInsts \gets \emptyset$
\For{each store instruction $si \in F.Instructions$}
  \State $sourceSet \gets BwSliceFindDef(si,si.source)$
  \State $destSet \gets FwSliceFindUse(si, si.dest)$
  \If{$candConfDesc \cap sourceSet \not = \emptyset$ \\ 
     AND $candHIDDesc \cap destSet \not = \emptyset$}
     \State $targetInsts \gets  targetInsts \cup \{si\}$
  \EndIf
\EndFor
\end{algorithmic}
\caption{}
\label{fig:algfintarget}
\end{figure}
